Foresight: planning future perception in streaming VLMs without retraining

Existing streaming vision-language models (VLMs) continuously perceive and reason over visual streams, but their computational pathways remain fixed throughout inference. Consequently, they cannot adapt computation to evolving scene dynamics, where different future events demand different levels and forms of perception. We show that streaming VLMs inherently possess the ability to anticipate the immediate future, and leverage this capability to dynamically configure future computation in a training-free manner. Realizing such anticipatory computation, however, is very challenging: future anticipation must be sufficiently reliable to guide computation, planning must run concurrently with streaming inference, and online reconfiguration must incur negligible overhead. To address these challenges, we introduce FORESIGHT, a dual-stream architecture comprising two Siamese LLMs with shared weights, input encoders, and KV cache. The first LLM continuously processes incoming tokens, while the second runs ahead of the stream to anticipate future context, plan future computation, and generate task responses without interrupting streaming inference. Each plan decides when to reason next, what to check then, and how densely to sample, keeping transient evidence separate from persistent control. The resulting computation plan is executed online through an efficient reconfiguration protocol with schemaguided decoding and lightweight diff-based updates, enabling dynamic adaptation with low overhead. With a frozen Qwen3-VL-8B backbone, FORESIGHT achieves 23.0 mean joint F1 on OmniPro Online evaluation beating strongest trained baseline by 9.5%, while improving the backbone by 6.7 on StreamingBench and 15.4 on OVO-Bench, with the largest gain of 18.7 when evidence arrives later in the video stream. Our source code will be made publicly available.

==> sections/related_work_iclr.tex <==
% ============================================================================
% ICLR Related Work section
%
% Requires in the main preamble:
%   \usepackage{booktabs}
%   \usepackage{amssymb}
%   natbib support (already provided by the standard ICLR template)
%
% If these macros are already defined elsewhere, remove the duplicates below.
% ============================================================================
\newcommand{\cmark}{\ensuremath{\checkmark}}
\newcommand{\pmark}{\ensuremath{\circ}}
\newcommand{\xmark}{--}

\section{Related Work}
\label{sec:related-work}

\paragraph{Streaming Video Understanding and Proactive Interaction.}
The transition from offline VideoLLMs to continuously operating assistants
requires models to process causally arriving observations and determine when an
interaction is warranted. VideoLLM-online
\citep{chen2024videollmonline} introduced the LIVE formulation, temporally
interleaving video and language and learning an EOS-based silence decision for
online interaction. MMDuet \citep{wang2025videollm} similarly reformulates
video--language interaction as a temporal ``duet,'' allowing textual responses
to be inserted while the video continues to unfold. LION-FS
\citep{li2025lionfs} separates a fast response-determination path from a slower,
higher-fidelity generation path, dynamically routing visual information to
balance real-time responsiveness and response quality.

A second line of work explicitly decouples streaming perception from response
generation. Dispider \citep{qian2025dispider} disentangles perception,
decision, and reaction: a lightweight streaming module continuously monitors
the video and triggers an asynchronous interaction module when a response is
needed. StreamBridge \citep{wang2025streambridge} equips offline VideoLLMs with
a compressed streaming memory and a decoupled activation model for proactive
response. StreamMind \citep{ding2025streammind} instead introduces an
event-gated cognition mechanism that invokes expensive language reasoning only
when its learned gate detects task-relevant events. ProAssist
\citep{zhang2025proactive} studies proactive assistance in egocentric streams,
combining a synthetic streaming-dialogue corpus with an end-to-end assistant
trained to generate contextually appropriate interventions. Eyes Wide Open
\citep{zhang2025eyeswideopen} further studies ego-streaming proactive
interaction through just-in-time response supervision and dynamic visual
compression. Together, these approaches establish that a streaming assistant
must reason not only about \emph{what} to output, but also about
\emph{when} interaction should occur.

Foresight operates at a different control level. Rather than treating the
streaming decision primarily as a response/silence trigger, each reasoning step
constructs a future-directed control state that determines how subsequent
inference should proceed. In particular, the planner determines when reasoning
should resume and what unresolved evidence should be checked when it does,
while perception continues to update the causal state.


\paragraph{Response Timing, Readiness, and Full-Duplex Streaming.}
Several recent methods improve the decision of when sufficient information has
arrived. LiveStar \citep{yang2025livestar} introduces Streaming Verification
Decoding (SVeD), using the compatibility of newly arriving evidence with the
existing response to determine whether another decode is necessary.
LiveStarPro \citep{yang2026livestarpro} extends this framework to long-horizon
streams with streaming causal training and tree-structured hierarchical memory,
jointly addressing response timing, incremental alignment, and long-term
forgetting. QueryStream \citep{zhang2026querystream} takes a complementary,
training-free approach: Query-Aware Differential Pruning removes visual tokens
that are both temporally redundant and weakly relevant to the user query, while
Relevance-Triggered Active Response schedules output using query relevance and
information density.

StreamReady \citep{azad2026streamready} makes evidence sufficiency itself the
central problem, learning a readiness mechanism that determines whether enough
supporting evidence has been observed to answer at the current time.
Proact-VL \citep{yan2026proactvl} similarly targets proactive real-time
interaction, jointly considering response latency, response timing, and output
quantity for interactive assistants. MiniCPM-o~4.5
\citep{cui2026minicpmo45realtimefullduplex} addresses a related but distinct
systems challenge through Omni-Flow, temporally multiplexing visual, audio, and
generated streams within a unified model to support full-duplex perception and
speech while repeatedly deciding whether to speak.

These systems primarily answer variants of \emph{should I respond now?} or
\emph{how can perception and response proceed efficiently together?}
Foresight additionally addresses what should happen when the answer is
\emph{not yet} ready: the current causal state specifies a future reasoning
horizon and a deferred verification objective. Thus, response readiness is one
component of the control plan rather than the complete control policy.


\paragraph{Anticipatory Planning and Streaming Reasoning.}
The closest prior work to our anticipatory motivation is StreamAgent
\citep{yang2025streamagent}. StreamAgent predicts future temporal intervals and
spatial regions likely to contain task-relevant evidence, constructs
reactive, proactive, and speculative plans, and can redirect subsequent
perception toward the anticipated evidence. It therefore establishes that
future information should actively influence streaming perception rather than
merely determine whether the current frame warrants a response.

Foresight shares this premise but uses a different abstraction. We do not
require explicit generation of multiple future trajectories or selection among
candidate plans. Instead, the current causal state produces the compact control
plan $\pi_t=(s_t,u_t)$, whose persistent component directly configures the
model's own subsequent inference. It specifies the interval before reasoning
resumes, carries an explicit unresolved question into that future step, and can
expose the same control interface to future perception density. Anticipation is
therefore represented as persistent state feedback over successive reasoning
steps.

Recent work has also investigated reasoning concurrently with a continuing
stream. Video Streaming Thinking (VST)
\citep{guan2026videostreamingthinking} introduces a watch-and-think paradigm in
which reasoning is performed during video playback and is learned through
streaming-specific supervised and reinforcement-learning post-training.
R3-Streaming \citep{liu2026r3streaming} formulates streaming inference as a
cascaded control problem over memory compression, answer readiness, and compute
routing, using reinforcement learning to allocate different reasoning
capabilities. Asynchronous Reasoning
\citep{yakushev2026asynchronousreasoningtrainingfreeinteractive} provides a
training-free mechanism for overlapping input, private reasoning, and public
generation through different positional views over shared LLM state.

Our focus is complementary to these approaches. Foresight does not primarily
optimize model routing or overlap language token streams; instead, a frozen
multimodal model becomes the controller of its own future reasoning schedule.
Continuous perception maintains the causal state, while the planning process
selects when that state should next be reconsidered and what uncertainty the
next reasoning step should resolve.


\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.08}
\caption{
\textbf{Positioning of Foresight relative to closely related streaming
methods.}
\cmark{} denotes an explicit component of the method,
\pmark{} denotes a partial or adjacent capability, and \xmark{} indicates that
the capability is not a central mechanism. ``Verification target'' refers to a
persistent representation of \emph{what the next reasoning step should
resolve}, rather than only a response-trigger condition.
}
\label{tab:related_comparison}
\begin{tabular}{lcccccc}
\toprule
\textbf{Method}
&
\textbf{\shortstack{Proactive\\timing}}
&
\textbf{\shortstack{Future-directed\\planning}}
&
\textbf{\shortstack{Schedules next\\reasoning}}
&
\textbf{\shortstack{Persistent\\verification target}}
&
\textbf{\shortstack{Adaptive\\perception}}
&
\textbf{\shortstack{Concurrent / decoupled\\stream processing}}
\\
\midrule

VideoLLM-online
& \cmark & \xmark & \xmark & \xmark & \xmark & \pmark \\

Dispider
& \cmark & \xmark & \xmark & \xmark & \xmark & \cmark \\

StreamBridge
& \cmark & \xmark & \xmark & \xmark & \pmark & \pmark \\

StreamMind
& \cmark & \xmark & \xmark & \xmark & \pmark & \cmark \\

LiveStarPro
& \cmark & \xmark & \xmark & \xmark & \xmark & \pmark \\

QueryStream
& \cmark & \xmark & \xmark & \xmark & \cmark & \xmark \\

StreamReady
& \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\

MiniCPM-o~4.5
& \cmark & \xmark & \xmark & \xmark & \xmark & \cmark \\

VST
& \pmark & \xmark & \xmark & \xmark & \xmark & \cmark \\

StreamAgent
& \cmark & \cmark & \pmark & \pmark & \cmark & \pmark \\

\textbf{Foresight}
& \cmark & \cmark & \cmark & \cmark & \cmark$^{\dagger}$ & \cmark \\
\bottomrule
\end{tabular}

\vspace{1mm}
\raggedright
\footnotesize
$^{\dagger}$Adaptive perception is exposed by the Foresight control interface and used in
our runtime illustrations; the lockstep quantitative benchmark reported in the
main experiments holds visual sampling rate fixed.
\end{table*}


\paragraph{Streaming Memory and Efficient Perception.}
The control problem is complementary to work on maintaining an efficient causal
representation of long streams. StreamChat \citep{liu2024streamchat} updates
the visual context during decoding through a cross-attention-based streaming
architecture, while ReKV \citep{di2025rekv} stores and retrieves query-relevant
video KV caches to decouple streaming analysis from later question answering.
StreamForest \citep{zeng2025streamforest} organizes observations into persistent
event-level memory structures for bounded long-term retention. Other approaches
reduce visual computation directly: CoPE-VideoLM
\citep{sarkar2026copevideolm} exploits codec motion vectors and residuals, while
Mage-VL \citep{yang2026magevlefficientcodecnativestreaming} uses codec-native
signals to allocate visual tokens preferentially to informative regions.
QueryStream similarly demonstrates that query-conditioned pruning can remove
substantial visual redundancy before it reaches the language model.

These methods primarily determine \emph{what information should be retained or
encoded}. Foresight is orthogonal: it determines \emph{when high-level
reasoning should occur and what future evidence that reasoning should seek}.
Efficient token selection, codec-native perception, or hierarchical memory can
therefore be combined with the same future-directed control loop.


\paragraph{Evaluation of Online and Proactive Understanding.}
StreamingBench \citep{lin2024streaming} evaluates continuously arriving
video through real-time, contextual, and proactive tasks. OVO-Bench
\citep{li2025ovobenchfarvideollmsrealworld} further distinguishes backward
tracing, real-time understanding, and forward active responding, explicitly
requiring models to defer answers until sufficient evidence becomes available.
OmniPro \citep{zhao2026omniprocomprehensivebenchmarkomniproactive} extends this
setting to omni-modal proactive interaction, where both semantic correctness
and response timing contribute to system quality. These benchmarks motivate our
view that streaming intelligence requires more than causal context maintenance
or response triggering: the inference process itself must adapt as the
information state evolves.

